Dimension-free Mixing for High-dimensional Bayesian Variable Selection

Yang et al. (2016) proved that the symmetric random walk Metropolis--Hastings algorithm for Bayesian variable selection is rapidly mixing under mild high-dimensional assumptions. We propose a novel MCMC sampler using an informed proposal scheme, which we prove achieves a much faster mixing time that is independent of the number of covariates, under the same assumptions. To the best of our knowledge, this is the first high-dimensional result which rigorously shows that the mixing rate of informed MCMC methods can be fast enough to offset the computational cost of local posterior evaluation. Motivated by the theoretical analysis of our sampler, we further propose a new approach called "two-stage drift condition" to studying convergence rates of Markov chains on general state spaces, which can be useful for obtaining tight complexity bounds in high-dimensional settings. The practical advantages of our algorithm are illustrated by both simulation studies and real data analysis.

==> LIT revision/preamble.tex <==
%%% math environments
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\theoremstyle{definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{conjecture}{Conjecture}
\newtheorem{assumption}{Assumption}
\newtheorem{condition}{Condition}

%%% math macros
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Cor}{\mathrm{Cor}}
\newcommand{\Gap}{\mathrm{Gap}}
\newcommand{\expit}{\mathrm{expit}}
\newcommand{\logit}{\mathrm{logit}}

\DeclareMathOperator*\argmin{arg\,min}
\DeclareMathOperator*\argmax{arg\,max}
\DeclareMathOperator*\trace{trace}
\DeclareMathOperator*\diag{diag}

\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\OPnorm}{\lVert}{\rVert_{\mathrm{op}}}
\DeclarePairedDelimiter{\FBnorm}{\lVert}{\rVert_{\mathrm{F}}}
\DeclarePairedDelimiter{\Onorm}{\lVert}{\rVert_{1}}
\DeclarePairedDelimiter{\Tnorm}{\lVert}{\rVert_{2}}
\DeclarePairedDelimiter{\Pnorm}{\lVert}{\rVert_{p}}
\DeclarePairedDelimiter{\Infnorm}{\lVert}{\rVert_{\infty}}

\newcommand{\ind}{\mathbbm{1}}
\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}
\newcommand{\sGamma}{\mathsf{\Gamma}}
\newcommand{\sTheta}{\mathsf{\Theta}}
\newcommand{\sLambda}{\mathsf{\Lambda}}
\newcommand{\sXi}{\mathsf{\Xi}}
\newcommand{\sPi}{\mathsf{\Pi}}
\newcommand{\sSigma}{\mathsf{\Sigma}}
\newcommand{\sPhi}{\mathsf{\Phi}}
\newcommand{\sPsi}{\mathsf{\Psi}}
\newcommand{\sOmega}{\mathsf{\Omega}}


\newcommand{\bA}{\bm{A}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\sA}{\mathsf{A}}
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\fA}{\mathfrak{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\sL}{\mathsf{L}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\sW}{\mathsf{W}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\bZ}{\bm{Z}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\sZ}{\mathsf{Z}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\fZ}{\mathfrak{Z}}


==> LIT revision/two_stage_proof.tex <==

\subsection{Path splitting for $(\sX_t)$} \label{sec:proof.split}
We first find a decomposition of $\bP$. 
Define a transition kernel $\bQ$   by 
\begin{equation*}\label{eq:def.Q}
\bQ(x,  \sC) =  \frac{ \bP(x,  \sC \cap \sA)   }{  \bP(x, \sA) }, \quad \forall \, x \in \sA, \, \sC \in \cE. 
\end{equation*}
The case $x \notin \sA$ is irrelevant to our proof, and one can 
simply let $\bQ(x, \cdot ) =\bP(x, \cdot)$  if $x \notin \sA$.
For $x \in \sA$, the distribution $\bQ(x, \cdot)$ is just $\bP(x, \cdot)$ conditioned on the chain staying in $\sA$. 
Further, condition~\eqref{d5}  implies that $(1 - q) \bQ(x,  \cdot )  \leq \bP(x, \cdot )$.
Hence, there always exists a ``complementary'' transition kernel $\bR$  such that 
\begin{equation}\label{eq:def.cP}
\bP(x,  \cdot ) = q \bR(x, \cdot ) +  (1 - q) \bQ(x, \cdot),  \quad \forall \,  x  \in \cX. 
\end{equation}

Now we re-construct the Markov chain $(\sX_t)_{t \in \bbN}$. 
First, we generate a sequence of i.i.d. Bernoulli random variables,  $(Z_0, Z_1,   \dots)$, such that $Z_i$ is equal to $1$ with probability $q$.  
Starting with $\sX_0 = x \in \cX$, we update the chain as follows. 
\begin{align*}
 \text{If } \sX_t \in \sA^c,    \quad & \text{ generate } \sX_{t + 1} \sim \bP(\sX_t, \cdot).  \\
 \text{If } \sX_t \in \sA, \,  Z_{t + 1}  = 0,    \quad & \text{ generate } \sX_{t + 1} \sim \bQ(\sX_t, \cdot). \\
 \text{If } \sX_t \in \sA, \, Z_{t + 1}  = 1,   \quad & \text{ generate } \sX_{t + 1} \sim \bR(\sX_t, \cdot). 
\end{align*}
It follows from~\eqref{eq:def.cP} that marginally, $(\sX_t)_{t \in \bbN}$ is a Markov chain with transition kernel $\bP$, and we will use $\P_x$ to denote the corresponding probability measure. 
Let $(\cF_t)_{t \in \bbN} = \sigma(\sX_0, \dots, \sX_t, Z_0, \dots, Z_t)$ denote the filtration generated by $(\sX_t, Z_t)_{t \in \bbN}$. Set $\omega_0 = 0$ and then  define the following hitting times with respect to $(\cF_t)$ recursively:
\begin{align*}
\sigma_k  =  \min\{ t \geq  \omega_{k - 1} \colon  \sX_t \in \sA \}, \quad \quad  \omega_k   =  \min\{ t > \sigma_k \colon  Z_t = 1 \}, 
\quad \quad k = 1, 2, \dots. 
\end{align*}
Observe that $\sX_t \in \sA$ if  $\sigma_k \leq t \leq \omega_k - 1$. 
For $k \geq 1$, $\omega_k$ marks the $k$-th time we update the chain using $\bR$, and then we return to the set $\sA$ at time $\sigma_{k + 1}$.  
Note that $\sigma_{k + 1} = \omega_k$ if $\sX_{\omega_k} \in \sA$ (i.e., the ``return'' happens immediately.)
For $k \geq 1$, let $S_{ k -1} =   \sigma_k  - \omega_{k - 1} \geq 0$ and $N_k =  \omega_k - \sigma_k \geq 1$. 
We have 
\begin{equation}\label{eq:s0}
\omega_k  = S_0 +  ( N_1 + S_1 ) + \cdots  + ( N_{k - 1} + S_{k - 1} ) + N_k. 
\end{equation}
  $N_k$ (resp. $S_{k - 1}$) can be seen as the length of  the $k$-th stay of $(\sX_t)$ in $\sA$ (resp. $\sA^c$). 
See Figure~\ref{fig.path} for a graphical illustration of our path splitting scheme. 

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.95\linewidth]{fig1.pdf} \\
\caption{An example of the evolution of $(X_t, Z_t)$. For $(X_t)$, we only indicate whether it is in $\sA$ or not. 
For $t = 5$ and $t = 8$, we generate $X_t$ from $\bR(X_{t - 1}, \cdot)$. 
Since $X_5 \in \sA$, $\omega_1 = \sigma_2 = 5$. 
For this example, we have $S_0 = 2$, $N_1 = 3$, $S_1 = 0$, $N_2 = 3$ and $S_2 = 2$. }\label{fig.path}
\end{center}
\end{figure}  
  
\subsection{Tail bound for $\tau^* $}  \label{sec:proof.tail}

Let $\sB_k =  \{ \sX_t \neq x^*,  \; \text{ for }   \sigma_k \leq t  \leq \omega_k - 1 \}$ be the event that $(\sX_t)$ does not hit $x^*$ during its $k$-th  stay in $\sA$. Then, for every fixed $t$, 
\begin{align*}
\P_x(    \tau^*  > t \geq \omega_k  ) \leq  \P_x(    \tau^*   \geq \omega_k  ) =  \P_x(  \sB_1 \cap   \cdots \cap \sB_k   ),
\end{align*}
since by $\omega_k$, $(\sX_t)$ has finished  $k$ ``excursions'' in $\sA$. 
%As in~\citet[Theorem 1]{rosenthal1995minorization},  we apply the union bound \tcr{(JY: this is not the union bound?)} to get 
As in~\citet[Theorem 1]{rosenthal1995minorization},  we apply the union bound to get 
\begin{equation}\label{eq:th1.union}
\begin{aligned}
\P_x (  \tau^* > t )  \leq \;& \P_x ( \omega_j > t) 
+ \P_x (  \tau^* > t , \omega_j \leq t)    \\
\leq \;& \P_x (    \omega_j  > t )  +   \P_x\left(  \sB_1 \cap   \cdots \cap \sB_j   \right), 
\end{aligned}
\end{equation}
which holds for any positive integer $j$. Therefore, it suffices to bound the two terms $\P_x (    \omega_j  > t )$ and $ \P_x\left(  \sB_1 \cap   \cdots \cap \sB_j   \right)$. The upper bound for $ \P_x\left(  \sB_1 \cap   \cdots \cap \sB_j   \right)$ is deferred to the next subsection. 
 
The key to bounding the tail probability $\P_x (    \omega_j  > t )$ is to show that  $S_0, N_1, S_1, \dots$ all have geometrically decreasing tails, and thus so does $\omega_j$. 
First, note that  $N_k =  \min \{  i  \geq 1 \colon Z_{\sigma_k + i} = 1 \}$, which is just a geometric random variable since $(Z_t)$ is an i.i.d. sequence. 
Therefore, $\E[ u^{ N_k  } ]$ exists for any $u < (1 - q)^{-1}$. 
We choose 
\begin{equation*}\label{eq:def.u}
u = \frac{1}{ 1 - q/2}, 
\end{equation*}
which is less than $\min\{ \lambda_1^{-1}, \lambda_2^{-1} \}$  by condition~\eqref{d5}. 
It is also evident by construction that $N_k$ is  independent of $\cF_{\sigma_k }$, which yields
\begin{equation}\label{eq:th1.N}
  \E_x [ u^{ N_k  } \mid  \cF_{\sigma_k} ]  =  \frac{ u q}{1  - u (1  - q)} = 2, \quad \text{a.s.} 
\end{equation}

Next, consider the random variables $\{S_k \colon k = 0, 1, \dots \}$. We have 
\begin{equation}\label{eq:th1.S0}
\E_x[  u^{S_0}  ] \leq  \E_x[  \lambda_1^{ - S_0}  ] \leq V_1(x), 
\end{equation}
by Lemma~\ref{lm:drift0} and drift condition~\eqref{d1}. 
Similarly,  for $S_k$ with $k \geq 1$,  
\begin{equation}\label{eq:th1.Sk}
\begin{aligned}
\E_x[  u^{S_k} \mid \cF_{\omega_k - 1} ]    \leq \;&  \E_x[ V_1(\sX_{\omega_k} )  \mid \cF_{\omega_k - 1} ]  \\ 
= \;&  \E_x[ V_1(\sX_{\omega_k} )  \mid \cF_{\omega_k - 1}, \sX_{\omega_k} \in \sA ] \P_x(  \sX_{\omega_k} \in \sA \mid   \cF_{\omega_k - 1}) \\
 & + \E_x[ V_1(\sX_{\omega_k} )  \mid \cF_{\omega_k - 1}, \sX_{\omega_k} \in \sA^c ] \P_x(  \sX_{\omega_k} \in \sA^c \mid   \cF_{\omega_k - 1}) \\ 
\leq \;&  \bR(  \sX_{\omega_k - 1},  \sA) + \frac{M}{2} \bR(  \sX_{\omega_k - 1},  \sA^c) 
%\P_x(  \sX_{\omega_k} \in \sA \mid   \cF_{\omega_k - 1}) + \frac{M}{2} \P_x(  \sX_{\omega_k} \in \sA^c \mid   \cF_{\omega_k - 1}) 
\leq M / 2, \quad \text{a.s.} 
\end{aligned}
\end{equation}
The second last inequality follows from  condition~\eqref{d3}  and the observation that  $\sX_{\omega_k}$ is generated from $\bR (\sX_{\omega_k - 1}, \cdot)$ and $\sX_{\omega_k - 1} \in \sA$. 
Using~\eqref{eq:s0},~\eqref{eq:th1.N},~\eqref{eq:th1.S0},~\eqref{eq:th1.Sk} and conditioning on  $\cF_{\omega_j - 1}, \cF_{\sigma_j}, \dots, \cF_{\sigma_1}$ recursively (which is allowed since $\omega_k - \sigma_k \geq 1$), we find that 
\begin{equation}\label{eq:th1.gf}
\E_x[  u^{ \omega_j  }  ]  = \E_x[ u^{ S_0 + \cdots + N_j } ]
\leq  2 V_1(x)     M^{j - 1}. 
\end{equation}
The tail probability $ \P_x (    \omega_j  > t ) $ then can be bounded by Markov's inequality. 


\subsection{Upper bound for $\P_x( \sB_1 \cap \cdots \cap \sB_j)$}  \label{sec:proof.prob}
Next, we show that  $\P_x( \sB_k \mid \sB_1, \dots, \sB_{k - 1} )\le \rho$ for some $\rho<1$, which implies the upper bound $\P_x (\sB_1 \cap \cdots \cap \sB_j ) \leq  \rho^j$. First, note that $(\sX_t, Z_t)$ forms a bivariate Markov chain and thus 
\begin{align*}
\P_x \left( \sB_k  \mid  \sX_{\sigma_k} =  y, \, Z_{ \sigma_k } =  z   \right)  =  \P_y (   \tau^* \geq  \omega_1 \mid Z_0 = z   ) =  \P_y (   \tau^* \geq  \omega_1),  \quad \text{a.s.} 
\end{align*}
where $\omega_1 = \min\{t \geq 1 \colon Z_t = 1 \}$ because $y = \sX_{\sigma_k} \in \sA$. 
Moreover, $\omega_1 = N_1$ is a geometric random variable independent of $\cF_0$. Conditioning on $N_1$, we find 
\begin{align}
\P_y (   \tau^* \geq  \omega_1) = \P_y (    \tau^* \geq    N_1  ) \nonumber  
 = \;&    \sum\limits_{t = 1}^\infty \P_y ( \tau^* \geq  t \mid  N_1  = t ) (1 - q)^{t - 1} q \nonumber \\ 
 = \;&   \sum\limits_{t = 1}^\infty \P_y (  \tau^* \geq  t \mid  Z_0 = \cdots = Z_{t - 1} = 0 ) (1 - q)^{t - 1} q,  \label{eq:py}
\end{align}
where in the last step we have used that $Z_t$ is independent of $(\sX_0, \dots, \sX_{t - 1})$  and thus the event $\{\tau^* \geq  t\}$. 
On the event $\{ Z_0 = \cdots = Z_{t - 1} = 0 \}$, $(\sX_0, \dots, \sX_{t -1})$ is a Markov chain with transition kernel $\bQ$.  
For $x \in  \sA \setminus \{x^*\}$,  let $q_x = \P(x, \sA^c)$ and  write   
\begin{align*}
(\bP V_2) (x)   =\;&  (1 - q_x)  (\bQ V_2)(x)  +  q_x \,  \E_x[ V_2(\sX_1) \mid \sX_1 \in \sA^c] . 
\end{align*}
Since $(\bP V_2) (x) \leq \lambda_2 V_2(x)$ for some $\lambda_2 < 1$,  we have $(\bQ V_2)(x) \leq  \lambda_2  V_2(x)$  by condition~\eqref{d4}. 
This drift condition enables us to apply Lemma~\ref{lm:drift0} and obtain from~\eqref{eq:py} that 
\begin{equation*}
   \P_y (    \tau^* \geq    N_1  )   \leq    \sum_{t = 1}^\infty   \lambda_2^t V_2(y)   (1 - q)^{t - 1} q    
=   \frac{ V_2(y)  \lambda_2  q }{1 - \lambda_2  (1 - q)}, 
\end{equation*}
for $y \in \sA$. 
Since $\lambda_2, q \in (0, 1)$ and $ K \geq  \sup_{y \in \sA} V_2(y)$, 
\begin{equation}\label{eq:def.rho}
\sup_{y \in \sA}   \P_y (    \tau^* \geq    N_1  )  \leq  \frac{ q  K   }{1 - \lambda_2 } \coloneqq \rho. 
\end{equation}
Note that $\rho  < 1$ by condition~\eqref{d5}. 
By conditioning on $\cF_{ \sigma_k}$, we find that $\P_x( \sB_k \mid \sB_1, \dots, \sB_{k - 1} )$ is also bounded by $\rho$, and thus $\P_x (\sB_1 \cap \cdots \cap \sB_j ) \leq  \rho^j$. 
 
\subsection{Generating function for  $\tau^*$} \label{sec:proof.gf}
We now combine the previous results to bound the generating function of $\tau^*$. Using the upper bound given in~\eqref{eq:th1.union} and  $\P_x (\sB_1 \cap \cdots \cap \sB_j ) \leq  \rho^j$,  we have 
\begin{align*}
\E_x[ \alpha^{-\tau^*}  ]  = \;&  1 + (\alpha^{-1} - 1) \sum_{k=0}^\infty \P( \tau^* > k ) \alpha^{-k} \\
\leq \;&  1 + (\alpha^{-1} - 1) \sum_{k=0}^\infty   \alpha^{-k} \left[ \rho^{j_k} + \P_x ( \omega_{j_k} > k   )  \right],
\end{align*}
for any $\alpha \in (0, 1)$, where $\rho$ is as given in~\eqref{eq:def.rho}. 
We choose $j_k =\lfloor rk + 1\rfloor \geq rk$ for some $r > 0$.
It then follows from~\eqref{eq:th1.gf} and~\eqref{eq:def.rho} that 
\begin{align*}
\E_x[ \alpha^{- \tau^*}  ]  \leq  1 + (\alpha^{-1} - 1) \sum_{k=0}^\infty  \alpha^{-k} \left[ \rho^{r k} + \frac{2 V_1(x)}{  M} \frac{    M^{r k} }{   u^k }  \right]. 
\end{align*}
The right-hand side  might diverge  if either $\rho^{r}$ or $M^{r}/u$ is too large. 
Hence, to obtain the optimal convergence rate, we set 
\begin{align*}
r = \frac{ \log u}{ \log (M / \rho) }, \quad \text{ which yields }
   \rho^{r} = \frac{ M^r }{u} < 1. 
\end{align*}
Since $M/2 \geq 1$, $0 < \rho < 1$ and $1 < u < 2$, we always have $r  \in (0, 1)$.

 
Finally, we choose $\alpha = (1 + \rho^r ) / 2 < 1$ and find that 
\begin{align*}
\E_x[ \alpha^{-\tau^*}  ]  \leq  1 +   \left(1 + \frac{ 2V_1(x) }{   M } \right) \frac{1 - \alpha}{\alpha - \rho^r} = 2 + \frac{2V_1(x)}{M}. 
\end{align*} 
The proof is then completed by applying Theorem~\ref{th:j2}. 

